Obfuscating IoT Device Scanning Activity via Adversarial Example Generation

Nowadays, attackers target Internet of Things (IoT) devices for security exploitation, and search engines for devices and services compromise user privacy, including IP addresses, open ports, device types, vendors, and products.Typically, application banners are used to recognize IoT device profiles during network measurement and reconnaissance. In this paper, we propose a novel approach to obfuscating IoT device banners (BANADV) based on adversarial examples. The key idea is to explore the susceptibility of fingerprinting techniques to a slight perturbation of an IoT device banner. By modifying device banners, BANADV disrupts the collection of IoT device profiles. To validate the efficacy of BANADV, we conduct a set of experiments. Our evaluation results show that adversarial examples can spoof state-of-the-art fingerprinting techniques, including learning- and matching-based approaches. We further provide a detailed analysis of the weakness of learning-based/matching-based fingerprints to carefully crafted samples. Overall, the innovations of BANADV lie in three aspects: (1) it utilizes an IoT-related semantic space and a visual similarity space to locate available manipulating perturbations of IoT banners; (2) it achieves at least 80\% success rate for spoofing IoT scanning techniques; and (3) it is the first to utilize adversarial examples of IoT banners in network measurement and reconnaissance.

==> material.tex <==


\clearpage



\section{Adversarial example}




\subsection{Vector}




This process is called word embedding, aiming at representing the ideal semantic space of words in a real-valued continuous vector space [59].
The commonly used embedding methods are one-hot, n-gram [60], and word2vec [61]. One-hot encoding is a technique whose dimension is equal to the size of the whole vocabulary, thus often resulting in large, very sparse vectors [62]. An n-gram model is a kind of probabilistic language model to predict next word in the form of previous words, which lacks long range dependency. Word2vec offers the best representation within a low dimensional semantic space learning from raw texts [63]. It includes two  architectures: continuous bag-of-words (CBOW) and skip-gram.
Word2vec is the most frequently used method for word embedding at present.



\subsection{Defense}


Deep neural networks (DNNs) are large neural networks whose architecture is organized as a series of layers of neurons, each of which serves as the individual computing units. Neurons are connected by links with different weights and biases and transmit the results of its activation function on its inputs to the neurons of the next layer.


Robustness. A robust DNN should not change its output as a result of small changes in its input. Hence, the prediction of the adversarial example x' should be y rather
than y 0 in a robust model, i.e., F(x 0 ) = y . Defense methods for enhancing the robustness of models are to increase the tolerance of $\varepsilon$ , making DNNs perform properly.



Since the problem of adversarial examples is so serious, a question arises: why adversarial examples exist in DNNs?

Researchers have been exploring the existence of adversarial examples since they were discovered.
Nowadays, there are two main points about their existence.
One is due to the \textbf{linear structure of DNNs}, which can lead to false predictions with a high probability.
Goodfellow et al. claimed that the primary cause of adversarial examples was the linear nature of DNNs.
Although the non-linear activation functions are the main parts of DNNs, they are linear in a sense.
Some of the main activation functions are shown, including tanh, sigmoid, relu, and ELU, where these functions are very piecewise linear.
Besides, there also exist other linear structures, such as the connection of each layer and convolution calculation.
A defect of the linear structure is that classification is still possible as it moves away from the decision boundaries, even though there is no training data. However, false predictions are usually made in these places, so that the presence of adversarial examples may be for this reason.
The other interpretation is that adversarial examples are generated based on \textbf{non-robust features of the data}.
Ilyas et al. [68] claimed, “adversarial vulnerability is a direct result of our
models sensitivity to well-generalizing features in the data.”
Through a series of experiments, they draw the conclusion that adversarial examples are not bugs, but features.
The features for prediction can be classified as robust and non-robust, if they exist in standard classification tasks.
Both of them are used for predicting the truth label which is pre-defined. But small perturbations can be added on non-robust features to make the final prediction incorrect.

Adversarial attacks are designed to degrade the performance of DNNs. Therefore, evaluating the effectiveness of the attack is based on the performance metrics of
different tasks.

\subsection{Metrics}





\begin{equation}\label{equ:metric:L}
  \|\Delta c\| =\sqrt[p]{\sum_{i=1}^{n}|c_i'-c_i|^p}
\end{equation}
where $\Delta c$ represents the perturbations. $c_i'$ and $c_i$ are the i-th factors in n -dimensional vectors.
Formula~\ref{equ:metric:L} represents a series of distances, where $p$ could be 0, 2, $\infty$, and so on.

L0 distance evaluates the number of changed pixels before and after modifications. It seems like edit distance, but it does not directly work in texts. Results of altered words in texts are varied. Some of them are similar to original words and the others may be contrary, even though the L0 distances of them are equal.
L2 represents the Euclidean distance. The original Euclidean distance is the beeline from one point to another in Euclidean space.
As the mapping of image, text, or others to this space, it acts as a metric to calculate the similarity between two objects, which are represented as the vectors.
L$\infty$ distance measures the maximum change.

Apart from imperceptibility, a good adversarial example in texts must convey the same semantic meaning with the original one, so that metrics are required to ensure this case.
Euclidean Distance. For two given word vectors $\overrightarrow{m}= (m_1, m_2,...,m_k)$ and $\overrightarrow{n}= (n_1, n_2,...,n_k)$  , the Euclidean
distance of them is shown in formula~\ref{equ:metric:eld}:
\begin{equation}\label{equ:metric:eld}
  D(\overrightarrow{m}, \overrightarrow{n}) = \sqrt{(m_1-n_1)^2 + ...+ (m_k-n_k)^2}
\end{equation}
where $m_i$ and $n_i$ are the i-th factors in the k -dimensional vectors respectively. The lower the distance is, the more similar they are. But Euclidean distance is more frequently used in image domain with a generalized term called L2 norm or L2 distance.

Cosine Distance.
Cosine distance is also a computational method for semantic similarity. It calculates the cosine value of the angle between two vectors. Compared with Euclidean distance, the cosine distance pays more attention to the difference between the directions of two vectors. The more consistent their directions are, the more similar they are.
For two given word vectors $\overrightarrow{m}$ and $\overrightarrow{n}$, the cosine similarity of them is shown in formula~\ref{equ:metric:cos}:
\begin{equation}\label{equ:metric:cos}
  D(\overrightarrow{m}, \overrightarrow{n}) = \frac{\overrightarrow{m} *\overrightarrow{n}}{\|\overrightarrow{m}\| * \|\overrightarrow{n}\|}
  = \frac{\sum_{i=1}^{k}m_i*n_i}{ \sqrt{\sum_{i=1}^{k}m_i^2} *\sqrt{\sum_{i=1}^{k}n_i^2} }
\end{equation}

Jaccard Similarity Coefficient. For two given sets A and B, their Jaccard similarity coefficient J(A, B) is shown in formula~\ref{equ:metric:jcd}:
\begin{equation}\label{equ:metric:jcd}
  J(A, B) = |A \bigcap B| / |A \bigcup B|
\end{equation}
where 0 $\leq$ J(A,B) $\leq$ 1. It means that the closer the value of J(A,B) is to 1, the more similar they are.

Edit Distance.
Edit distance is a way to measure the minimum modifications by turning a string to another. The lower it is, the more similar the two strings are.
It can be applied to computational biology and natural language processing. Levenshtein distance is also known as edit distance with insertion, deletion, replacement operations.


These metrics are applied to different objects.
Among them, Euclidean distance, cosine distance, and WMD are used on vectors. Adversarial examples and the original ones in texts are transformed into vectors, and then these three methods are applied to calculate the distance between the
vectors.
On the contrary, Jaccard similarity coefficient and edit distance are directly used on text inputs without the need to convert raw texts to vectors.




\subsection{DNN}

Deep neural networks (DNNs) are large neural networks whose architecture is organized as a series of layers of neurons, each of which serves as the individual computing units. Neurons are connected by links with different weights and biases and transmit the results of its activation function on its inputs to the neurons of the next layer.
A deep neural network (we use DNN and deep learning model interchangeably hereafter) can be simply presented as a nonlinear function $f_\theta$: $\textbf{X} \rightarrow \textbf{Y}$,  where X is the input features/attributes, Y is the output predictions that can be a discrete set of classes or a sequence of objects.
$\theta$ represents the DNN parameters and are learned via gradient-based back-propagation during the model training.
Best parameters would be obtained by minimizing the gap between the model's prediction $f_\theta(\textbf{X})$  and the correct label Y, where the gap is measured by loss function $J(f_\theta(\textbf{X}),Y)$.

Apart from the feed forward neural networks and Convolutional Neural Networks (CNN), Recurrent/Recursive Neural Networks (RNN) and their variants are the most common neural networks used in NLP, because of their natural ability of handling sequences.


\emph{Feed Forward Networks}. Feed-forward network, in particular multi-layer perceptrons (MLP), is the simplest neural network. It has several forward layers and each node in a layer connects to each node in the following layer, making the network fully connected. MLP utilizes nonlinear activation function to distinguish data that is not linearly separable. MLP works with fixed-sized inputs and do not record the order of the elements. Thus it is mostly used in the tasks that can be formed as supervised learning problems.
The major drawback of feed forward networks in NLP is that it cannot handle well the text sequences in which the word order matters.


\emph{Convolutional Neural Network} contains convolutional layers and pooling (down-sampling) layers and final fully-connected layer. Activation functions are used to connect the down-sampled layer to the next convolutional layer or fully-connected layer.
CNN allows arbitrarily-sized inputs. Convolutional layer uses convolution operation to extract meaningful local patterns of input. Pooling layer reduces the parameters and computation in the network and it allows the network to be deeper and less-overfitting.
Overall, CNN identifies local predictors and combines them together to generate a fixed-sized vector for the inputs, which contains the most or important informative aspects for the application task.
Word2Vec represent words as input. Then the convolutional operation is limited to the direction of word sequence, rather than the word embeddings. Multiple filters in pooling layers deal with the variable length of sentences.

\emph{Recurrent Neural Networks} are neural models adapted from feed-forward neural networks for learning mappings between sequential inputs and outputs. RNNs allows data with arbitrary length and it introduces cycles in their computational graph to model efficiently the influence of time.
The model does not suffer from statistical estimation problems stemming from data sparsity and thus leads to impressive performance in dealing with sequential data.
Bi-directional RNN thus was proposed for looking at sentences in both directions, forwards and backwards, using two parallel RNN networks, and combining their outputs.
Since RNN is a natural choice to model various kinds of sequential data, it has been applied to many NLP tasks. Hence RNN has drawn great interest for adversarial attack.

RNN has many variants, among which Long Short-Term Memory (LSTM) network gains the most popularity.
LSTM is a specific RNN that was designed to capture the long-term dependencies. In LSTM, the hidden state are computed through combination of three gates, i.e., input gate, forget gate and output gate, that control information flow drawing on the logistic function. LSTM networks have subsequently proved to be more effective than conventional RNNs.

\emph{Sequence-to-sequence learning (Seq2Seq)} is one of the important breakthroughs in deep learning and is now widely used for NLP applications.
Seq2Seq model has the superior capacity to generate another sequence information for
a given sequence information with an encoder-decoder architecture.
Usually, a Seq2Seq model consists of two recurrent neural networks: an encoder that processes the input and compresses it into a vector representation, a decoder that predicts the output.
Latent Variable Hierarchical Recurrent Encoder-Decoder (VHRED) model is a recently popular Seq2Seq model that generate sequences leveraging the complex dependencies between subsequences.


\textbf{Perturbations} are intently created small noises that to be added to the original input data examples in test stage, aiming to fool the deep learning models.
\begin{equation}\label{equ:perb}
\begin{aligned}
  x'    & =    x + \eta, \quad f(x) = y, x \in  X \\
  f(x') & \neq y,  \quad  or \quad f(x') = y', \quad y' \neq y
\end{aligned}
\end{equation}
where $\eta$ is the worst-case perturbation.



i) evaluating the deep neural networks by fooling them with unperceivable perturbations;
ii) intentionally changing the output of the deep neural networks;
and iii) detecting the oversensitivity and over-stability points of the deep neural networks and finding solutions to defense the attack.


\subsection{Transferability}

Transferability is a common property for adversarial examples. It reflects the generalization of the attack methods. Transferability means adversarial examples generated for one deep neural network on a dataset can also effectively attack another deep neural network (i.e., cross-model generalization) or dataset (i.e., cross-data generalization). This property is more often exploited in black-box attacks as the details of the deep neural networks does not affect the attack method much. It is also shown that untargeted adversarial examples are much more transferable than targeted ones [ 83 ]. Transferability can be organized into three levels in deep neural networks: (1) same architecture with different data; (2) different architectures with same application; (3) different architectures with different data [ 154 ]. Although current works on textual attacks cover both three levels, the performance of the transferred attacks still decrease drastically compared to it on the original architecture and data, i.e., poor generalization  ability. More efforts are expected to deliver better generalization ability.

\textbf{Automation}

Some reviewed works are able to generate adversarial examples automatically, while others cannot. In white-box attacks, leveraging the loss function of the DNN can identify the most affected points (e.g., character, word) in a text automatically. Then the attacks are performed on these points by automatically modifying the corresponding texts. In black-box attacks, some attacks, e.g. substitution train substitute DNNs and apply white-box attack strategies on the substitution. This can be achieved automatically. However, most of the other works craft the adversarial examples in a manual manner. For example, [ 55 ] concatenated manually-chosen meaningless paragraphs to fool the reading comprehension systems, in order to discover the vulnerability of the victim DNNs. Many research works followed their way, not aiming on practical attacks, but more on examining robustness of the target network. These manaul works are time-consuming and impractical. We believe that more efforts in this line could pass through this barrier in future.



\subsection{IoT Limitations}


Encrypted vs Unencrypted Network Traffic : Some fingerprinting
approaches do not need access to the packet payload, i.e. they can
work on both encrypted and unencrypted packets. Conversely, others
are designed to work on encrypted and unencrypted packet payloads,
such as the algorithm proposed by Robyns et al. [ 40 ] which exploits
per-bit entropy analysis (MAC address randomization). Furthermore,
some approaches are able to extract the features required only if the
payload is not encrypted.


private protocols.


Hardware Feature vs Software Feature Fingerprinting : The for-
mer approach uses features that are extracted using special Physical
Unclonable Function (PUF) circuits to capture hardware-intrinsic
properties. The latter approach uses behavioural software properties,
which could be found in the network traffic generated by the IoT
device.


Static Feature vs Dynamic Feature Fingerprinting : A static fea-
ture fingerprinting includes only features that do not usually change
over the time (e.g. MAC address), while dynamic feature finger-
printing uses dynamic features that can change over time such as
inter-arrival time associated with data flow.


Hardware Feature vs Software Feature Fingerprinting : The for-
mer approach uses features that are extracted using special Physical
Unclonable Function (PUF) circuits to capture hardware-intrinsic
properties. The latter approach uses behavioural software properties,
which could be found in the network traffic generated by the IoT
device.


Adaptive vs Fixed Fingerprinting Algorithms : An “adaptive” fin-
gerprinting approach uses an algorithm that changes in response to
certain conditions observed during the fingerprinting process. On the
other hand, when the fingerprinting process always uses the same
(deterministic) algorithm with pre-determined and constant parame-
ters for all cases observed, we can consider that as “fixed”.


Real Devices vs Simulated : Fingerprinting approaches based on
deep-learning algorithms require a large amount of data to properly
identify devices. Moreover, budget constraints do not allow for a
large number of devices to produce an exhaustive dataset for eval-
uation purposes. Thus, tools to simulate IoT devices are used (e.g.
Node-RED [ 25 ]). In this case, traffic flows and most of the important
features of typical categories of IoT devices – such as fridges or
washing machines – can be simulated and used to build datasets. On
the other hand, if real devices are used, the results will be more rep-
resentative of real-world scenarios, but the budgetary requirements
are higher as well.



Testbed vs Real World Evaluation : Fingerprinting approaches are
developed either on testbeds or in real-world environments. The
latter approaches provide additional resilience and deployment cred-
ibility for the fingerprinting algorithm.



\section{materials}


The model-based approach has three stages: a preprocessing module, a word embedding module, and a classification module.
Given a banner of a host, the preprocessing module convert it to textual tokens, and vectorizing module further convert it into vectors as the input of models.
DNNs are large neural networks whose architecture is organized as a series of layers of neurons, each of which serves as the individual computing units. Neurons are connected by links with different weights and biases and transmit the results of its activation function on its inputs to the neurons of the next layer.


Perturbation method: replace the important word and randomly add a word before or after this word. The exact method depends on the partition.\\
% 修改方法：替换重点词并在这个词的前或后随机添加一个词。具体方法视分区而定。
\begin{itemize}
         \item \emph{Visual focus areas(VFA)}

         Original word:$w$, Substitute word:$w_1$.

         The characters within $w$ are first inverted to the inverted $w_r$ of the original $w$. Unicodes  are added to the periphery of $w_r$: U+202D, U+2066, U+202E, U+2069,U+202C. They are all invisible and serve the purpose: to make the words that have been inverted display positively. This operation does not have any visual impact and the words are still visually normal and unaltered.\\

         % 原词Original word：w
        % 替换词Substitute word：w1。先将w内字符反转为原来w的倒序wr。在wr的外围加上三对Unicode U+202D U+2066 U+202E wr U+202C U+2069 U+202C。他们都是不可见的，其作用是：使已经被反转的单词正向显示。这个操作不会带来任何视觉上的影响，视觉上还是正常的，没有被改动过的词。

         inserted word $w_2$:among other classes of spelling similar focus words, a word with the greatest cosine similarity was chosen.

         Replace $w$ with $w_1$ and randomly insert $w_2$ before or after $w_1$, and make the inserted $w_2$ invisible with the help of Unicode U+0008. This also does not have any visual impact, the inserted word is not visible to the human eye, but the inserted $w_2$ further reduces the model effect.


        % 添加的词w2。在其他类拼写相似的重点词中，选择一个余弦相似度最大的词。

        % 用w1代替w，并随机将w2差入到w1之前或之后，并将插入的w2借助Unicode U+0008将插入的w2隐去。这也不会带来任何视觉上的影响，人眼无法看到插入的词，但插入的w2会增加攻击的成功率。

        \item \emph{Visual sub-focus areas(VSFA)}

        Original word: $w$, Substitute word:$w_1$.

        Select a character at random in $w$ and replace the selected character with a visually similar character. This operation introduces a small amount of visual impact.
                % 原词Original word：w
        % 替换词Substitute word：w1。在w中随机选择一个字符，将选中的字符用视觉上相似的字符替换。这个操作会带来少量的视觉上的影响。

        inserted word $w_2$: among other classes of spelling similar focus words, a word with the greatest cosine similarity was chosen.\\
         Replace $w$ with $w_1$ and randomly insert $w_2$ before or after $w_1$, and make the inserted $w_2$ invisible with the help of Unicode U+0008.

        % 添加的词w2。在其他类拼写相似的重点词中，选择一个余弦相似度最大的词。

        % 用w1代替w，并随机将w2差入到w1之前或之后，并将插入的w2借助Unicode U+0008将插入的w2隐去。

        \item \emph{Non-visual focus areas(NVFA}

        Original word: $w$, Substitute word:$w_1$.

        among other classes of spelling similar focus words, a word with the greatest cosine similarity was chosen.\\
         inserted word $w_2$:same to $w_1$.\\
         Replace $w$ with $w_1$ and randomly insert $w_2$ before or after $w_1$, and make the inserted $w_2$ invisible with the help of Unicode U+0008.
         % 原词Original word：w
        % 替换词Substitute word：w1。在其他类拼写相似的重点词中，选择一个余弦相似度最大的词。

        % 添加的词w2。与w1相同

        % 用w1代替w，并随机将w2差入到w1之前或之后，并将插入的w2借助Unicode U+0008将插入的w2隐去。
        \item \emph{Invisible areas(IVA)}

         Original word: $w$, Substitute word:$w_1$.

         among other classes of spelling similar focus words, a word with the greatest cosine similarity was chosen.

         inserted word $w_2$:same to $w_1$.

         Replace $w$ with $w_1$ and randomly insert $w_2$ before or after $w_1$, which does not need to be hidden because it is an invisible part.
         % 原词Original word：w
        % 替换词Substitute word：w1。在其他类拼写相似的重点词中，选择一个余弦相似度最大的词。

        % 添加的词w2。与w1相同

        % 用w1代替w，并随机将w2差入到w1之前或之后，因为是不可见部分，所以不用隐去。
\end{itemize}


Why should the visible part use visual substitution and cosine similarity substitution when the reverse does not cause any visual impact?
% 既然翻转不会造成任何视觉上的影响，为什么可见部分还要使用视觉替换和拼写相似的余弦相似度替换呢？


Data that has been perturbed by four separate partitioning methods is becoming less and less reversible. This means that it is increasingly difficult for a malicious adversary to recover the original data from the data defended by our method and to classify it correctly. Because Unicode scrambling is more regular, an adversary who scans for the appropriate Unicode can process the sample according to the Unicode's role and thus recover the data. In contrast, visually similar characters have a one-to-many characteristic, and it is difficult to complete the cross-reduction with a single rule. It is necessary to use human or OCR to correspond visually similar characters to the original characters, but there are many similar characters, and it is very difficult to find them artificially and cover them all. The words replaced by cosine similarity are difficult to find in the pre-processing process and can also perturb the model better.
% 分别经过四个分区的修改方法扰动过的数据，可还原程度是越来越低的。也就是说恶意的对手想要从经过我们方法防御的数据中还原原本的数据并正确分类是越来越难的。因为Unicode的扰动较为规则化，对手如果扫描到了相应的Unicode就可以根据Unicode的作用处理样本从而还原数据。而视觉相似的字符存在一对多的特性，用单一的规则很难完成对照还原，需要借助人为或OCR将视觉相似字符与原字符对应的方式，但是相似的字符有很多，人为寻找十分困难且难以全部覆盖。而采用余弦相似度替换的词很难在预处理过程中被发现，也能更好的扰动模型。



Why are the added words in the invisible area not hidden but the added words in the NVFA area are hidden?
% 为什么不可见部分的添加词不隐藏而NVFA区域中的添加词隐藏了？


Unicode perturbations are more regular, and the adversary can process the sample according to the role of Unicode if the corresponding Unicode is scanned in order to recover the data. For example, visually hidden characters can be removed directly, and reversed strings can be reversed to their original form. Therefore, keeping the insertions unhidden in the invisible region makes it more difficult for a malicious adversary to recover the data, so that our approach maintains some protection against Unicode scrambling and visual scrambling if the adversary can recover them all.
% Unicode的扰动较为规则化，对手如果扫描到了相应的Unicode就可以根据Unicode的作用处理样本从而还原数据。比如将原来视觉上隐去的字符直接去除，将翻转的字符串翻转回原来的样子。所以，在不可见区域中保留插入词不隐去可以增加恶意对手还原数据的难度，是的我们的方法在对手可以将Unicode扰动和视觉扰动全部还原的情况下保持一定的防护能力。





\subsection{White-box Attack}


In white-box attack, the attack requires the access to the model's full information, including architecture, parameters, loss functions, activation functions, input and output data. White-box attacks typically approximate the worst-case attack for a particular model and input, incorporating a set of perturbations. This adversary strategy is often very effective.

\emph{FGSM-based.}
FGSM is Fast Gradient Sign Method, which is derived by following equation.
\begin{equation}\label{L-BFGS}
  \eta = \arg\min_{\eta}(\lambda\|\eta \|^2_{2} + J(x+\eta, y') )
\end{equation}
This equation~\ref{L-BFGS} is very effective, but highly expensive.
FGSM fixed size of $\eta$ and maximized the cost, as follows.
\begin{equation}\label{FGSM-1}
  \eta = \arg\max_{\eta}J(x+\eta, y); s.t. \|\eta\|_{\infty} \leq \epsilon
\end{equation}
Then they linearized the problem with a first-order Taylor series approximation, as follow.
\begin{equation}\label{FGSM-2}
  \eta = \arg\max_{\eta}J(x, y) + \eta^T\nabla_xJ(x,y); s.t. \|\eta\|_{\infty} \leq \epsilon
\end{equation}
We got the closed-form solution of $\eta$, as follow.
\begin{equation}\label{FGSM-3}
  \eta = \epsilon \cdot sign(\nabla_xJ(x,y))
\end{equation}
where $\epsilon$ is a parameter set by attacker, controlling the perturbation's magnitude.
$sign(x)$ is the sign function which returns 1 when $x > 0$, and -1 when $x < 0$, otherwise returns 0. $\nabla_xJ(x,y)$ denotes the gradient of loss function respect to the input, and can be calculated via back-propagation. 
 

